Two novel numerical methods for gradient flows: generalizations of the Invariant Energy Quadratization method

In this paper, we conduct an in-depth investigation of the structural intricacies inherent to the Invariant Energy Quadratization (IEQ) method as applied to gradient flows, and we dissect the mechanisms that enable this method to uphold linearity and the conservation of energy simultaneously. Building upon this foundation, we propose two methods: Invariant Energy Convexification and Invariant Energy Functionalization. These approaches can be perceived as natural extensions of the IEQ method. Employing our novel approaches, we reformulate the system connected to gradient flow, construct a semi-discretized numerical scheme, and obtain a commensurate modified energy dissipation law for both proposed methods. Finally, to underscore their practical utility, we provide numerical evidence demonstrating these methods' accuracy, stability, and effectiveness when applied to both Allen-Cahn and Cahn-Hilliard equations.

==> Errors_3.tex <==
\begin{tabular}{|c|c|c|c|c|c|c}
\hline
0.094215 & 0.047625 & 0.023729 & 0.011624 & 0.005532 & 0.002479 & 0.000956 \\ \hline
0.063632 & 0.032332 & 0.016092 & 0.007814 & 0.003635 & 0.001541 & 0.000513 \\ \hline
0.114006 & 0.057330 & 0.028529 & 0.014009 & 0.006720 & 0.003069 & 0.001247 \\ \hline
\end{tabular}



